Computing Execution Times with eXecution Decision Diagrams in the Presence of Out-Of-Order Resources

Worst-Case Execution Time (WCET) is a key component for the verification of critical real-time applications. Yet, even the simplest microprocessors implement pipelines with concurrently-accessed resources, such as the memory bus shared by fetch and memory stages. Although their in-order pipelines are, by nature, very deterministic, the bus can cause out-of-order accesses to the memory and, therefore, timing anomalies: local timing effects that can have global effects but that cannot be easily composed to estimate the global WCET. To cope with this situation, WCET analyses have to generate important over-estimations in order to preserve safety of the computed times or have to explicitly track all possible executions. In the latter case, the presence of out-of-order behavior leads to a combinatorial blowup of the number of pipeline states for which efficient state abstractions are difficult to design. This paper proposes instead a compact and exact representation of the timings in the pipeline, using eXecution Decision Diagram (XDD) [1]. We show how XDD can be used to model pipeline states all along the execution paths by leveraging the algebraic properties of XDD. This computational model allows to compute the exact temporal behavior at control flow graph level and is amenable to efficiently and precisely support WCET calculation in presence of out-of-order bus accesses. This model is finally experimented on the TACLe benchmark suite and we observe good performance making this approach appropriate for industrial applications.

==> xsteps.tex <==
\subsection{The timing semantic}

Similar to the \XG analysis, the analysis with the state vector should parse the instructions and stages following an order and update the state vector in that order to ensure the correctness of the state vector and the analysis. The order described in the Equation~\ref{eq:eval-order} is used.

Precisely, when analyzing an instruction to be executed on a stage:

\begin{enumerate}
    \item At the start of the instruction on the stage, the analysis computes the maximum of the release time (state) of all necessary resources with respect to the instruction and the stage because the instruction and the stage defines the \emph{USE} of resources. That maximum corresponds to the actual ready time of entering the stage;
    \item The state vector is \emph{updated} for sub-states recording the ready time of the instruction on the stage;
    \item The instruction starts to be executed in the stage, it takes some time to go through the stage i.e. plus of constant time independent of the state vector;
    \item The instruction is released from the stage, the state vector is \emph{updated} for sub-states recording this release time.
\end{enumerate}

However, the use behavior or the update behavior is not only stage dependent but also instruction dependent. For instance, the Memory Order should be considered only if the instruction performs memory related operations. To enable a flexible definition of the timing behavior, we define the \emph{timing step language} defining the timing behavior of instructions on the stages. Therefore, the timing behavior of an instruction on a stage is divided into several small steps: waiting for a resource, release a resource, or consuming a time. 


\begin{definition}
\begin{equation*}
    STEP = WAIT(\R)|RELEASE(\R)|CONSUME(\XDD)
\end{equation*}

A resource is composed by a state (several dates) $\XDD^{n}$, its wait behavior and its release behavior.
\begin{equation*}
    \R = \XDD^{n} \times f_{wait} \times f_{release}
\end{equation*}

The wait behavior $f_{wait}$ describes the effects when waiting for the resource: it computes the earliest start time due to this resource by considering the state of the resource.

The release behavior $f_{release}$ describes how the state vector is updated upon the release of the resource. 



\end{definition}

As the $f_{wait}$ and $f_{release}$ is related to the algebraic properties of state transition, we will define it later in the Section~?.


A \emph{step program} is a sequence of steps. Following the analysis behavior above, the timing behavior of an instruction on a stage can be systematically compiled into a \emph{step program} by considering (1) the acquiring resource before entering the stage (generating $WAIT$)(2) the releasing resources when ready to enter into the stage (generating $RELEASE$) (3) the time past in the stage (generating $CONSUME$), and (4) the releasing resources upon exiting the stage (generating $RELEASE$). 

An example of generation for ME stage is showed in the Figure~\ref{fig:timing-steps-generation}.
\begin{figure}[h]
    \centering
\begin{gather*}
    Gen(I/ME) = \\
    WAIT(ProgramOrder_{ME});\\
    WAIT(CapacityOrder_{ME});\\
    WAIT(PipelineOrder_{EX-ME});\\
    WAIT(QueueEffect_{ME-CM});\\
    WAIT(CapacityOrder_{ME}); \\
    if(I.useMemory) WAIT(MemoryOrder);\\
    if(I.useRegisters) WAIT(DataDependency(I.usedRegisters);\\
    \\
    RELEASE(ProgramOrder_{ME});\\
    RELEASE(QueueEffect_{EX-ME});\\
    \\
    CONSUME(I.latency); \\
    \\
    RELEASE(PipelineOrder_{ME-CM});\\
    RELEASE(CapacityOrder_{ME});\\
    if(I.useMemory) RELEASE(MemoryOrder);\\
    if(I.writeRegisters) RELEASE(DataDependency(I.writtenRegisters);)
\end{gather*}
    \caption{Timing steps generation of ME stage}
    \label{fig:timing-steps-generation}
\end{figure}

Thus, any instruction sequence can be compiled into a \emph{step program} by following the evaluation order defined in the Equation~\ref{eq:eval-order}. The timing step language brings two benefits:  (a) it simplifies the conversion of analysis model from high-level micro-architecture description. \footnote{In fact, in our framework OTAWA, the step program is automatically generated from high level description of the ISA and the micro-architecture.} (b) together with the algebraic properties of the analysis, it eases the creation of the computational model of the analysis that we will show in the following section.


